Development of physically based plastic flow rules for body-centered cubic metals with temperature and strain rate dependencies

In this Thesis we first show how the shape of the Peierls barrier and its dependence on the applied loading can be extracted from the data obtained in atomistic studies at 0 K. We consider the Peierls barrier as a two-dimensional periodic function of the position of the intersection of the dislocation line with the perpendicular {111} plane, with adjustable terms dependent on the shear stresses parallel and perpendicular to the slip direction. The functional forms of these terms are based on the effective yield criterion recently developed on the basis of atomistic modeling of the glide of screw dislocations at 0 K. The minimum energy path between two potential minima, and thus the corresponding activation barrier, is obtained using the Nudged Elastic Band method. The constructed Peierls barrier reproduces correctly both the well-known twinning-antitwinning asymmetry observed for pure shear parallel to the slip direction and the effect of shear stresses perpendicular to the slip direction. This advancement introduces for the first time the effect of both shear stresses parallel and perpendicular to the slip direction into the model of thermally activated dislocation motion. Based on this model we formulate a general yield criterion that includes not only the full stress tensor but also effects of temperature and strain rate. This approach forms a basis for multislip yield criteria and flow relations for continuum analyses in both single and polycrystals the results of which can be compared with experimental observations.

==> centralf.tex <==
\chapter{Plastic flow of bcc metals from central force potentials}
\label{chap_centralf}

\begin{flushright}
  People are like crystals. It is the defects in them that make them interesting. \\
  \emph{Sir F. Charles Frank}
\end{flushright}

For completeness, we will now look at the behavior of screw dislocations in certain bcc metals
investigated using central force potentials that do not include the directional bonding. The
question is which of the features of the dislocation behavior, if any, can be reproduced by these
simple potentials and what characteristics are purely products of the directional bonding. We will
be mainly interested in the structure of the dislocation core and its transformation under the
stress that is responsible for the twinning-antitwinning asymmetry and effect of shear stress
perpendicular to the slip direction.

%----------------------------------------------------------------------------------------------------
%----------------------------------------------------------------------------------------------------

\section{Simulations of Mo using the Finnis-Sinclair potential}

%----------------------------------------------------------------------------------------------------

\subsection{Structure of the dislocation core}

The $\gamma$-surface calculated using the Finnis-Sinclair potential for molybdenum predicts that
screw dislocations possess degenerate cores that is in contrast to BOP predicting the non-degenerate
cores. At zero applied stress, the core of an isolated screw dislocation can exist in any of the two
configurations plotted in \reffig{fig_core_MoFS} that we will further designate as core \lcore and
core \rcore. The two cores, each obeying the three-fold symmetry of the lattice, are related to one
another by an additional $[\bar{1}01]$ diad symmetry. 

Due to the unidirectional spreading of the core on the three $\gplane{110}$ planes of the $[111]$
zone, one can expect that the stress to move the dislocation ``to the right'' and ``to the left'' in
\reffig{fig_bl_core_MoFS} will not be identical. For example, when the shear stress parallel to the
slip direction is applied such that it acts ``to the right'', the \rcore core will require lower
energy to move because it is already spread on this plane in the direction of glide. For the same
orientation of shear, the \lcore core will need an appreciably larger stress because its
$(\bar{1}01)$ branch is extended in the opposite direction. Instead, it is natural to expect that
the \lcore core will move along either the $(0\bar{1}1)$ or the $(\bar{1}10)$ plane because the
other two branches are extended on these planes in the direction of applied shear. 

\begin{figure}[!htb]
  \centering
  \includegraphics[width=7cm]{fig/bl_core_MoFS-left} \hfill
  \includegraphics[width=7cm]{fig/bl_core_MoFS-right} \\
  a) \lcore core \hskip7cm b) \rcore core
  \parbox{14cm}{\caption{The degenerate dislocation core in Mo related by the vertical $[\bar{1}01]$
      diad calculated using the Finnis-Sinclair potential.}
    \label{fig_core_MoFS}}
\end{figure}

The fact that the two degenerate cores can coexist raises a possibility that a screw dislocation can
be composed of finite segments possessing cores of both types. If this is so, some parts of the
dislocation can have higher mobility because lower stress is needed for their motion. From this
point of view, it is therefore important to study the behavior of \emph{both} dislocation cores
under stress. This can be done in the very same way we studied the behavior of screw dislocations
using BOP, which will again provide us with the $\CRSS-\chi$ and $\CRSS-\tau$ dependencies
quantifying the influence of orientation of applied loading and shear stress perpendicular to the
slip direction.

%----------------------------------------------------------------------------------------------------

\subsection{Orientational dependence of the shear stress parallel to the slip direction}

Although the dislocation cores depicted in \reffig{fig_core_MoFS} are symmetric images of each
other, it does not guarantee that the two will behave identically under the applied stress. We will
again begin by studying the response of the dislocation to the pure shear stress parallel to the
slip direction acting in the MRSSP at angle $\chi$ relative to the $(\bar{1}01)$ plane, see
\reffig{fig_planes}. Depending on the type of core to be studied, the simulations always started
from the relaxed configuration in \reffig{fig_core_MoFS}. The applied shear, given by the stress
tensor (\ref{eq_tensor_sigma}), had been built up gradually in steps and the dislocation core
relaxed before proceeding to the next higher stress. The critical stress at which the dislocation
moved into the next equivalent lattice site in the direction of applied stress, i.e. ``to the
right'', was identified as the CRSS for slip.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/CRSS_chi_MoFS-left.eps}
  \parbox{14cm}{\caption{Orientational dependence of shear stress parallel to the slip
      direction for the \lcore core.}
    \label{fig_CRSS_chi_MoFS-left}}
\end{figure}

The $\CRSS-\chi$ dependence obtained from loading the \lcore dislocation core by pure shear parallel
to the slip direction is plotted in \reffig{fig_CRSS_chi_MoFS-left} as circles. One can immediately
see that there is a significant twinning-antitwinning asymmetry in that the CRSS for positive $\chi$
is much larger than the CRSS corresponding to negative $\chi$. In antitwinning shear (i.e. at
positive $\chi$) the dislocation moves on the $(\bar{1}01)$ plane, while in twinning shear (at
negative $\chi$) the slip plane changes to $(0\bar{1}1)$. As we stated above, the unidirectional
character of spreading of the \lcore core should not allow the dislocation to move on the
$(\bar{1}01)$ plane ``to the right'' which seems to contradict \reffig{fig_CRSS_chi_MoFS-left}. By
closely looking at the transformation of the dislocation core before and after the first elementary
step, we observed that the \lcore core first significantly constricts on the $(\bar{1}01)$ plane and
extends on $(0\bar{1}1)$ and $(\bar{1}10)$ planes. At CRSS, the initially sessile \lcore dislocation
core flips into the \rcore configuration that is mobile in the $(\bar{1}01)$ plane owing to its
extended $(\bar{1}01)$ branch. This core flipping is expected to occur every time the stacking fault
energy of the other core becomes lower than the energy of the actual core configuration. In
contrast, no core flipping takes places at negative $\chi$ for which orientations $(0\bar{1}1)$
becomes the most highly stressed branch of the core. As a consequence, the dislocation readily
constricts on the $(\bar{1}01)$ and $(\bar{1}10)$ planes, which transforms the core into a form that
is glissile in the $(0\bar{1}1)$ plane.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/CRSS_chi_MoFS-right.eps}
  \parbox{14cm}{\caption{Orientation dependence of shear stress parallel to the slip
      direction for the \rcore core.}
    \label{fig_CRSS_chi_MoFS-right}}
\end{figure}

Considering the opposite \rcore core as the starting configuration, one arrives at the $\CRSS-\chi$
dependence plotted in \reffig{fig_CRSS_chi_MoFS-right} in which the data for pure shear parallel to
the slip direction are plotted as circles. In comparison to the \lcore core, the
twining-antitwinning asymmetry is now appreciably weaker and also the magnitude of the CRSS at
positive $\chi$ rises more quickly with the angle $\chi$ than we observed for the \lcore core in
\reffig{fig_CRSS_chi_MoFS-left}. This should not be surprising since the \rcore core is extended on
the $(\bar{1}01)$ plane in the direction of applied shear and, therefore, requires lower stress to
move. Furthermore, the actual slip plane for any orientation of the MRSSP is $(\bar{1}01)$ which is
again consistent with the structure of the \rcore dislocation core. The initially sessile core is
transformed by stress into its glissile form by constricting the two branches on $(0\bar{1}1)$ and
$(\bar{1}10)$ planes and extending in the slip plane. No core flipping is observed in this case
which implies that the stacking fault energy of the \rcore core is energetically favorable.

%----------------------------------------------------------------------------------------------------

\subsection{Loading in tension and compression}

Superimposed in \reffig{fig_CRSS_chi_MoFS-left} and \reffig{fig_CRSS_chi_MoFS-right} are also data
corresponding to uniaxial loadings along several characteristic directions spanning the
stereographic triangle $[001]-[011]-[\bar{1}11]$. Recall that this data can be used to decide
whether the shear stress parallel to the slip direction is the only relevant stress component that
affects the plastic flow of molybdenum or there is also a significant effect of shear stress
perpendicular to the slip direction.

In the case of the \lcore core, \reffig{fig_CRSS_chi_MoFS-left} shows that the $(\chi,\CRSS)$ data
for uniaxial loading are close to the values calculated from pure shear. This means that the shear
stress $\tau$, perpendicular to the slip direction, plays only a minor role in the motion of \lcore
dislocations and, therefore, the CRSS will be only a weak function of the magnitude of $\tau$. In
contrast, \reffig{fig_CRSS_chi_MoFS-right} reveals that there is appreciable difference between the
CRSS values calculated for pure shear and for uniaxial loading if the dislocation has initially the
\rcore type. One can therefore expect that shear stress perpendicular to the slip direction will
play an important role for dislocations possessing these cores.

%----------------------------------------------------------------------------------------------------

\subsection{Effect of shear stress perpendicular to the slip direction}

Since the dislocation core calculated from the Finnis-Sinclair potential for molybdenum is less
compact than the non-degenerate core obtained from BOP, the core transformations induced by the
shear stress perpendicular to the slip direction will have larger extent. The relaxed dislocation
cores corresponding to positive and negative applied $\tau$ are shown as dislocation displacement
maps in \reffig{fig_bl_tau0.05_MoFS}.

In \reffig{fig_bl_core_MoFS}, we have seen that the two variants of the unstressed dislocation core
are mutually related by the $[\bar{1}01]$ diad. The question now is, whether we can find any
relation between the structures of the two cores under the shear stress perpendicular to the slip
direction. Consider first the stress tensor (\ref{eq_tensor_tau}) applied in the coordinate system
where axis $y$ is the normal of the MRSSP $(\bar{1}01)$ and $z$ is parallel to the slip
direction. Notice that the $[\bar{1}01]$ axis now coincides with the $y$ axis of the coordinate
system and, simultaneously, the stress tensor is invariant with respect to $180\deg$ rotation around
this axis. Therefore, it comes at no surprise that even under the applied shear perpendicular to the
slip direction, the \lcore core is related to the \rcore by still the same $[\bar{1}01]$ diad
operation. This symmetry is shown for positive and negative shear stress $\tau$ in
\reffig{fig_bl_tau0.05_MoFS}.

If the MRSSP deviates from the $(\bar{1}01)$ plane, the $y$ axis of the coordinate system is no
longer identical to the $[\bar{1}01]$ diad. Because of the twinning-antitwinning asymmetry, one
cannot expect that the cores of \lcore and \rcore dislocations will be related by the same symmetry
as above. In this case, the rotation of the coordinate system about the $[\bar{1}01]$ diad axis
changes the orientation of the axis $y$ (and therefore also the orientation of the MRSSP) and thus
the two \lcore and \rcore configurations cannot be related by the $[\bar{1}01]$ diad. For example,
consider that the \rcore core is subjected to stress tensor (\ref{eq_tensor_tau}) that is defined in
the system $(\bar{3}12)[111]$, i.e. the angle of the MRSSP measured in the $[111]$ zone relative to
the $(\bar{1}01)$ plane is $\chi \approx +19\deg$. The $[\bar{1}01]$ diad operation flips the \rcore
core into the \lcore core and, simultaneously, rotates the coordinate system into
$(\bar{2}\bar{1}3)[\bar{1}\bar{1}\bar{1}]$, i.e. the angle of the MRSSP measured in the
$[\bar{1}\bar{1}\bar{1}]$ zone relative to the $(\bar{1}01)$ plane is still $\chi \approx
+19\deg$. Because $(\bar{3}12)$ and $(\bar{2}\bar{1}3)$ planes are distinguished by the
twinning-antitwinning asymmetry, the two cores cannot be mirror images of each other. This symmetry
holds only between the two cores calculated for MRSSPs with opposite angles $\chi$, as is shown
schematically in \reffig{fig_degcore_symm}. Consequently, if we consider a given applied stress
tensor (\ref{eq_tensor_tau}), one arrives at dislocation cores of the \lcore and \rcore type that
are related by the $[\bar{1}01]$ diad only if the angles $\chi$ for these two simulations have equal
magnitudes but \emph{opposite} signs, see \reffig{fig_degcore_symm}.

\begin{figure}[!htb]
  \centering
  \includegraphics{fig/degcore_symm}
  \parbox{12cm}{\caption{Schematic illustration of the symmetry between \rcore and \lcore
      dislocation cores calculated at the same applied shear $\tau$.}
  \label{fig_degcore_symm}}
\end{figure}

\begin{figure}[!p]
  \centering
  \includegraphics[width=7cm]{fig/bl_tau-0.05_MoFS-left.eps} \hskip1.5cm
  \includegraphics[width=7cm]{fig/bl_tau-0.05_MoFS-right.eps} \\
  a) \lcore core, $\tau/C_{44}=-0.05$ \hskip4.5cm b) \rcore core, $\tau/C_{44}=-0.05$ \\[1cm]
%
  \includegraphics[width=7cm]{fig/bl_tau+0.05_MoFS-left.eps} \hskip1.5cm
  \includegraphics[width=7cm]{fig/bl_tau+0.05_MoFS-right.eps} \\[1em]
  c) \lcore core, $\tau/C_{44}=+0.05$ \hskip4.5cm d) \rcore, $\tau/C_{44}=+0.05$
%
  \caption{Transformation of the dislocation core after applying pure negative (a,b)
  or positive (c,d) shear stress perpendicular to the slip direction. The stress tensor 
  (\ref{eq_tensor_tau}) is given in the coordinate system in which $x$ axis coincides with the 
  $(\bar{1}01)$ plane.}
    \label{fig_bl_tau0.05_MoFS}
\end{figure}

The effect of the shear stress perpendicular to the slip direction on the magnitude of the CRSS at
which the dislocation moves can again be quantified by the $\CRSS-\tau$ dependencies calculated for
several discrete orientations, $\chi$, of the MRSSP. Because of the degenerate character of the
dislocation core, we obtained two sets of dependencies corresponding to the two types of cores used
as starting configurations. For MRSSP $(\bar{1}01)$, these are plotted separately in
\reffig{fig_chi0_MoFS-left} and \reffig{fig_chi0_MoFS-right}.

One can see that the CRSS in \reffig{fig_chi0_MoFS-left} calculated for a dislocation with the
\lcore core is only weakly dependent on $\tau$, which we understood as an effect of the spreading of
the dislocation core on the $(\bar{1}01)$ plane \emph{against} the direction of applied shear. At
positive applied $\tau$, the dislocation core initially extends on both $(0\bar{1}1)$ and
$(\bar{1}10)$ planes because the shear stress exerted on these planes is identical. When the shear
stress parallel to the slip direction reaches the CRSS, the core flips into the \rcore configuration
and further moves on the $(\bar{1}01)$ plane. In contrast, at negative applied $\tau$, the
dislocation core moves entirely on the $(0\bar{1}1)$ and without any flipping into the \rcore
configuration. The reason why the core flips at positive $\tau$ and not at negative $\tau$ will be
analyzed in detail below.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/chi0_MoFS-left}
  \parbox{15cm}{\caption{Effect of shear stress perpendicular to the magnitude of the CRSS for the
  \lcore core of molybdenum (Finnis-Sinclair). The MRSSP is $(\bar{1}01)$.}
  \label{fig_chi0_MoFS-left}}
\end{figure}

Interestingly, the $\CRSS-\tau$ dependence for the \rcore core plotted in
\reffig{fig_chi0_MoFS-right} is very different to \reffig{fig_chi0_MoFS-left}. The slope of the data
reveals that CRSS for this type of core is very sensitive to the shear stress perpendicular to the
slip direction. At positive $\tau$, the dislocation moves by single slip on the  $(\bar{1}01)$ plane
which is not surprising owing to the spreading of the core on this plane in the direction of applied
shear. At larger negative $\tau$, the dislocation moves on the $(0\bar{1}1)$ plane which is
preceded by core flipping into the \lcore configuration.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/chi0_MoFS-right}
  \parbox{15cm}{\caption{Effect of shear stress perpendicular to the magnitude of the CRSS for the
  \rcore core of molybdenum (Finnis-Sinclair). The MRSSP is $(\bar{1}01)$.}
  \label{fig_chi0_MoFS-right}}
\end{figure}

Earlier in this chapter, we have prognosed that screw dislocations in molybdenum may involve
segments of both \lcore and \rcore types. In this case, the plastic deformation would take place
when the applied shear reaches the lower of the two CRSS values calculated for the two dislocation
cores. For example, at large positive values of $\tau$, the dislocation possessing the \rcore core
requires lower CRSS to move than the corresponding \lcore dislocation which needs additional stress
to flip its core. This preference reverses at negative $\tau$ for which the lower CRSS to move on
the $(0\bar{1}1)$ plane corresponds to the \lcore core, while the \rcore dislocation needs
an extra stress to flip its core.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/chi0_MoFS-both}
  \parbox{15cm}{\caption{Comparison of the $\CRSS-\tau$ dependencies for the MRSSP $(\bar{1}01)$
  calculated using BOP and from the Finnis-Sinclair potential. For a given value of $\tau$, the
  latter data are obtained by taking the lower of the two CRSS values calculated for the \lcore and
  \rcore core. The symbol $\rhd$ refers to the \rcore core extended ``to the right'' and the symbol
  $\lhd$ to the \lcore extended ``to the left''.}
  \label{fig_chi0_MoFS-both}}
\end{figure}

Yet another interesting information is obtained by investigating the conditions under which a
dislocation core flips into the other configuration. This flipping occured for the \lcore core at
positive $\tau$ and for the \rcore at negative $\tau$ which means that the other type of core is
energetically more favorable than the actual core. This is indeed proven by comparing the CRSS
values calculated for these two cores at positive and negative $\tau$. At negative $\tau$, the CRSS
for the \lcore is lower than the CRSS for the \rcore and the \lcore core thus have higher mobility
than the \rcore core. The opposite is true at positive $\tau$, where the CRSS for the \lcore is
larger than the CRSS for the \rcore, and the \rcore core is more mobile than the opposite \lcore
core.

%----------------------------------------------------------------------------------------------------
%----------------------------------------------------------------------------------------------------

\section{Simulations of Ta using the Finnis-Sinclair potential}



%----------------------------------------------------------------------------------------------------

\subsection{Structure of the dislocation core}

In contrast to molybdenum, the $\gamma$-surface for tantalum calculated using the Finnis-Sinclair
potential predicts that an isolated $1/2[111]$ screw dislocation in Ta possesses a non-degenerate
core which is consistent with the DFT studies of \citet{yang:01}. The dislocation core in Ta is
spread symmetrically on the three $\gplane{110}$ planes of the $[111]$ zone, as is shown in
\reffig{fig_core_TaFS}.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=7cm]{fig/bl_core_TaFS}
  \parbox{10cm}{\caption{The non-degenerate dislocation core in Ta calculated using the 
      Finnis-Sinclair potential.}
    \label{fig_core_TaFS}}
\end{figure}

The fact that Finnis-Sinclair potential for tantalum predicts a correct structure of the dislocation
core even without considering angular dependence of bonding raises an important question, whether
there are some other features of the behavior of screw dislocations in Ta that can be well
reproduced by central force potentials. In order to answer this question, one would first need to
construct the BOP as outlined in Chapter~\ref{sec_BOP}. The BOP for tantalum and niobium are now in
the last stage of development and the results of this type will be published in the future.

%----------------------------------------------------------------------------------------------------

\subsection{Orientational dependence of the shear stress parallel to the slip direction}

Starting with the relaxed dislocation core shown in \reffig{fig_core_TaFS}, we first applied shear
pure stress parallel to the slip direction applied in several discrete orientations of the
MRSSP. The dependence of the CRSS on the angle of the MRSSP is plotted as circles in
\reffig{fig_CRSS_chi_TaFS}. One can observe a significant twinning-antitwinning asymmetry in that
the CRSS for antitwinning shear (i.e. positive $\chi$) is always larger than for the twinning shear
(i.e. negative $\chi$).

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/CRSS_chi_TaFS.eps}
  \parbox{14cm}{\caption{Orientational dependence of shear stress parallel to the slip
      direction for tantalum (Finnis-Sinclair).}
    \label{fig_CRSS_chi_TaFS}}
\end{figure}

For negative and also intermedium positive angles $\chi$, the dislocation moves by elementary steps
on the $(\bar{1}01)$ and $(0\bar{1}1)$ plane which results in a macroscopic slip on the
$(\bar{1}\bar{1}2)$ plane. It is worthwhile noting, that the slip never proceeds by elementary steps
directly on the $(\bar{1}\bar{1}2)$ plane, which we will further emphasize by using the term zig-zag
slip. At large positive $\chi$, the dislocation does not move and, instead, develops a twin on the
$(\bar{2}11)$ plane and grows as the stress increases.

%----------------------------------------------------------------------------------------------------

\subsection{Loading in tension and compression}

Similarly as in the other simulations we performed before, also the $\CRSS-\chi$ dependence for
tantalum shown in \reffig{fig_CRSS_chi_TaFS} reveals a marked difference between the CRSS values
calculated for pure shear parallel to the slip direction and for uniaxial loading. This implies that
also the shear stress perpendicular to the slip direction plays a significant role in the plastic
deformation. 

%----------------------------------------------------------------------------------------------------

\subsection{Effect of shear stress perpendicular to the slip direction}

The stucture of the dislocation core obtained for positive and negative applied shear stress
perpendicular to the slip direction is plotted in \reffig{fig_tau0.05_TaFS}. Both cores are very
similar to those calculated for the non-degenerate core in molybdenum using BOP. At negative $\tau$,
the core constricts on $(0\bar{1}1)$ and $(\bar{1}10)$ planes which makes the dislocation more
mobile in the $(\bar{1}01)$ plane. On the other hand, at positive $\tau$ the core weakly constricts
on these two non-glide planes, which results in only marginal rearrangements relative to the
unstressed core in \reffig{fig_core_TaFS}.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=7cm]{fig/bl_tau-0.05_TaFS.eps} \hskip1.5cm
  \includegraphics[width=7cm]{fig/bl_tau+0.05_TaFS.eps} \\[1em]
  a) $\tau/C_{44}=-0.05$ \hskip6cm b) $\tau/C_{44}=+0.05$
  \caption{Transformation of the dislocation core after applying pure shear stress perpendicular
  to the slip direction. The stress tensor (\ref{eq_tensor_tau}) is given in the coordinate system 
  in which $x$ axis coincides with the $(\bar{1}01)$ plane. \todo{There seems to be some strange
  spreading of the core that I eliminated by erasing the arrows around the core that are not on the
  three $\gplane{110}$ planes.}}
    \label{fig_tau0.05_TaFS}
\end{figure}

In order to quantify the effect of the shear stress perpendicular to the slip direction on the
magnitude of the CRSS, we carried out atomistic simulations under stress in which we first applied
the shear stress perpendicular to the slip direction. For a completely relaxed block at the given
$\tau$, we subsequently kept $\tau$ constant and added the shear stress parallel to the slip
direction until the dislocation moved. The $\CRSS-\tau$ dependence obtained for shear stress
parallel to the slip direction applied in the MRSSP $(\bar{1}01)$ is plotted in
\reffig{fig_chi0_TaFS}.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=13cm]{fig/chi0_TaFS}
  \parbox{15cm}{\caption{Effect of shear stress perpendicular to the magnitude of the CRSS for the
  tantalum (Finnis-Sinclair). The MRSSP is $(\bar{1}01)$.}
  \label{fig_chi0_TaFS}}
\end{figure}

At positive $\tau$, the dislocation moves by single slip on the $(\bar{1}01)$ plane. The decreasing
tendency of the $\CRSS-\tau$ dependence is caused by progressively elongating the $(\bar{1}01)$
branch of the dislocation core with increasing shear stress perpendicular to the slip direction. At
$\tau\approx 0$ and negative values, the dislocation moves by zig-zag slip on the $(\bar{1}01)$ and
$(0\bar{1}1)$ planes which results in a macroscopic slip on the $(\bar{1}\bar{1}2)$ plane. However,
the motion at the atomistic level never proceeds directly on the $\gplane{211}$ plane but, instead,
by a zig-zag slip on the two $\gplane{110}$ planes.

